BOSS: Benchmark for Observation Space Shift in Long-Horizon Task

Robotics has long sought to develop visual-servoing robots capable of completing previously unseen long-horizon tasks. Hierarchical approaches offer a pathway for achieving this goal by executing skill combinations arranged by a task planner, with each visuomotor skill pre-trained using a specific imitation learning (IL) algorithm. However, even in simple long-horizon tasks like skill chaining, hierarchical approaches often struggle due to a problem we identify as Observation Space Shift (OSS), where the sequential execution of preceding skills causes shifts in the observation space, disrupting the performance of subsequent individually trained skill policies. To validate OSS and evaluate its impact on long-horizon tasks, we introduce BOSS (a Benchmark for Observation Space Shift). BOSS comprises three distinct challenges: "Single Predicate Shift", "Accumulated Predicate Shift", and "Skill Chaining", each designed to assess a different aspect of OSS's negative effect. We evaluated several recent popular IL algorithms on BOSS, including three Behavioral Cloning methods and the Visual Language Action model OpenVLA. Even on the simplest challenge, we observed average performance drops of 67%, 35%, 34%, and 54%, respectively, when comparing skill performance with and without OSS. Additionally, we investigate a potential solution to OSS that scales up the training data for each skill with a larger and more visually diverse set of demonstrations, with our results showing it is not sufficient to resolve OSS. The project page is: https://boss-benchmark.github.io/

==> sections/benchmark.tex <==
\section{The \bm Benchmark}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/bms.png} 
    \caption{This figure illustrates the three challenges of \bm where \pb occurs, with progressively increasing difficulty.\gb{Captions needs to be significantly expanded. I also feel like this figure does not look good. It has a lot of text and basic figures. Can you illustrate each challenge using concrete visual examples and fewer text? It would be more intuitive and look a lot better than the current figure. I also feel like the current figure has a lot going on in terms of arrows. You need to simplify it. For instance, I looked at it for ~30s and I still have no idea what some of these illustrations mean. Make it simpler and reduce the amount of text, arrows, and other potentially uncessary/overwhelming details}}
    \label{fig:bm_arch}
\end{figure*}




We introduce the \bm benchmark, designed to facilitate a comprehensive empirical study of the \pb problem across modern IL methods. To study this issue, we construct the environment (Section~\ref{subsec:bm_env}) using the Libero simulation platform~\cite{liu2024libero}. \bm includes three challenges (Section~\ref{subsec:bm_1}~\ref{subsec:bm_2}) designed not only to validate the existence of \pb but also to demonstrate its significant negative impact on the success of long-horizon tasks\gb{You also don't list any numbers overviewing your benchmark, which might be useful? How many tasks? How many trajectories, etc etc? From this overview, I don't have almost any idea what this benchmark looks like, what the scale of it is, etc.}. We also introduce four IL algorithms as baselines for evaluation on \bm (Section~\ref{subsec:basic_bl}). Additionally, we present a potential solution to \pb and the large-scale, diverse dataset generated as part of its preparation (Section~\ref{subsec:our_bl}).\gb{In my view, the solution shouldn't be a part of the benchmark section. It's not really related to the benchmark itself. Would it make sense to put it as another section?}


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.4\textwidth, height=0.2\textheight]{example-image} 
%     \caption{example for picked tasks from Libero-100}
%     \label{fig:picked_tasks}
% \end{figure}

\subsection{Environment}
\label{subsec:bm_env}
% Introduce:
% 1. The based Libero Environment: basic + task customization (intro bddl)
% 2. Obs space and action space, control freq ...

We build \bm on the Libero platform~\cite{liu2024libero}, which, although originally designed for lifelong robot learning tasks, provides diverse manipulation scenes featuring a Franka Emika Panda robot arm, a wide range of tasks, and high flexibility for creating and customizing tasks. These features make Libero an excellent foundation for developing \bm, enabling us to adapt it specifically to study the \pb problem.

From Libero-100, the most comprehensive and diverse task suite in Libero, we select all 44 skill-level tasks spanning 12 diverse manipulation scenes, encompassing a wide range of object interactions and motor skills, which we denote as \taskoriginal. To form our base task set, we exclude multi-skill tasks (e.g., ``open the top drawer of the cabinet and put the bowl in it'') and include only single-skill tasks (e.g., ``open the bottom drawer of the cabinet'').\gb{Why? It seems that those would be even better suited to study the OSS problem} All three challenges are constructed from this refined set.\gb{Do we need a figure to highlight the main properties of the benchmark? Since this is one of our main contributions, I think it would be great to showcase that as a figure, especially if we want to emphasize particular things about the benchmark, i.e., a large number of tasks, etc?}
% , with selected examples shown in Fig.~\ref{fig:picked_tasks}.

For consistency, we define the observation space as a combination of third-person camera images, 7-DoF robot arm joint angles, and 2-DoF parallel gripper joint states. The action space is defined as a 7-dimensional relative Cartesian displacement (w.r.t. the gripper frame), and the control frequency is set to 20 Hz.\gb{Does this need to fo in the environment section? Seems like it breaks the flow of the benchmark description. This to me seems more fitting to some implementations details section}


\yy{For all challenges, May need to improve many statements to be more concise and accurate using math annotations when problem definition is improved.}

% \begin{table}[h!]
% \centering
% \caption{Language Examples Description of benchmark tasks in BM1, BM2, and BM3. \textcolor{red}{might delete later if we wanna add BMs language descriptions in Fig.2.}}
% \label{tb:bm_examples}
% \begin{tabular}{llll}
% \hline
%       & BM1 & BM2 & BM3 \\ \hline
% Exm-1 &     &     &     \\ \hline
% Exm-2 &     &     &     \\ \hline
% Exm-3 &     &     &     \\ \hline
% Exm-4 &     &     &     \\ \hline
% Exm-5 &     &     &     \\ \hline
% \end{tabular}
% \end{table}


\subsection{Challenge 1: Single-Step Modification\gb{Maybe Single-Step State Modification? From this name it's not clear what you are actually modifying}}
\label{subsec:bm_1}
% Intro - osm problem is incurred by transition between skills, so we for sure need to study how much effect the single-step modification can bring on the next skill.
% Briefly introduce bddl file - How I use it to create modification?
% metric - performance drop (PD).

% As discussed in Section~\ref{sec:problem_definition}, \pb occurs when skill-irrelevant environmental elements are altered in a manner that do not impact the dynamic preconditions of the next skill (i.e., the next skill is still physically capable of being completed), but do violate the visual preconditions. 

\gb{The section structure of this seems disjoint. You go from environment to Challenge 1 without any explanation or overview. Maybe instead you could have a separate section dedicated to all the challenges and then just list each challenge as a subsection? Also, before introducing each challenge maybe you could provide a brief overview of what each challenge entails? Right now the transition between the previous section and this section seems very abrupt and not very intuitive}

As discussed in Section~\ref{sec:problem_definition}, \pb occurs when skill-irrelevant predicates are altered in a manner that do not impact the completeness of current skill, but do disrupt the visuomotor skill policy execution.\gb{The writing of this sentence is somewhat cumbersome and difficult to follow. Maybe you could rewrite it to be more clear. Also, I'd encourage you to include concrete examples to illustrate this so that no reader would have any doubts about what you are trying to say with your verbal descriptions. Also, as I mentioned, it would be great if your figure illustrating three challenges included some visual examples. Then you could also reference to that figure in this text when reminding what the first challenge is} In the context of skill chaining, a foundational structure in long-horizon tasks, the preceding skill is the most likely source of \pb for the subsequent skill\gb{I don't fully understand what it means for the skill to be a source of OSS. I feel like the writing is unclear and ambiguous}. Therefore, we introduce a challenge, \bma, specifically designed to evaluate the impact of \pb caused by single-step transitions on the performance of baseline methods (see examples in Figure~\ref{fig:bm_arch}).

To investigate the impact of single-step \pb on baseline methods, we compare their performance on the next skill without \pb and with \pb\gb{Again this could be made more clear with some examples}. For the former, we evaluate baselines on tasks from \taskoriginal. For the latter, we modify tasks from \taskoriginal to simulate \pb caused by the preceding skill.\gb{I feel like your descriptions of this is confusing, at least to me. I don't know why we have to mention BOSS-44 at all. You can just say that we evaluate each method on each of the 44 tasks in a scenario where OSS exists and in a scenario where it doesn't. It's easy to understand that. I'm also generally confused why you even need this BOSS-44? It adds another name to keep track of and I personally don't understand how is this different than BOSS? Can we just have one name BOSS without creating these additional names, which there are already a lot of (e.g., three challenges, etc.) so that it would be easier for the reader to keep track of all of these details} Libero's customization flexibility plays a crucial role here, as its task environments are generated using Planning Domain Definition Language (PDDL) files\notezlf{you may mention PDDL when introducing task planning in formulation? you can mention it defines e.g., operators, and what you need to modify here}. This allows us to easily add new objects (e.g., placing a potato in a bowl or on a tabletop) or modify object states (e.g., closing an opened drawer). These modifications enable us to simulate single-step \pb efficiently and evaluate baseline performance on the altered tasks.

To quantify the impact of \pb, we introduce the metric ``\textbf{Performance Drop (PD)},'' defined as the difference between the success rate of a baseline on the original skill-level task and its success rate on the task with single-step \pb\notezlf{I don't think it's necessary to create these kind of abbreviations in general, people may get confused and this term not used much in your paper. If you really need, maybe explain in table title. Also, a better name may be performance delta, as it may be positive or negative}.\gb{I feel like this should go into the experimental section, next to the definition of evaluation metrics, not here}



\subsection{Challenge 2: Accumulated Modification\gb{Again, i feel like the challenge names could be more intuitive and self-explanatory}}
\label{subsec:bm_2}
Along a skill chain, \pb can occur in multiple skills\gb{can you give an example?}, with these modifications accumulating and affecting the current skill. Thus, it is valuable to study the differences between accumulated \pb and single-step \pb. To address this, we introduce another challenge, \bmb, specifically designed to analyze the impact of \pb accumulation across preceding skills (check examples in Figure~\ref{fig:bm_arch}). \gb{from this paragraph, to me it's not clear at all what this accumulation is referring to}

Similar to \bma, we evaluate baseline performance on the next skill under two conditions: without \pb and with accumulated \pb. Using PDDL description files, we create two sets of modified tasks: one with two modifications and another with three modifications\gb{why is such setup used? Seems like these are arbitrary choices}. However, multiple modifications can sometimes conflict. For example, a modification such as ``place an apple inside the small bowl'' could conflict with another that specifies ``place a potato inside the small bowl,'' potentially causing the Libero environment to break due to overlapping space constraints. To address this, we develop a \textbf{Rule-based Automatic Modification Generator (RAMG)} to ensure compatibility and scalability when generating modifications for a single task. We provide details of RAMG in Section~\ref{subsec:our_bl}. We use the same metric \textbf{PD} as \bma to measure the impact of accumulated \pb.\gb{It would be great to provide a detailed list of modifications that your system can implement. Similarly, for completenes/reporducibility, it would be great to provide a list of all the tasks included in your dataset along with the numbers for each task. This would emphasize the benchmark contribution and also make the paper more reproducible. Right now many details about your benchmark/dataset are missing.}




\subsection{Challenge 3: Real Long-Horizon Task}
\label{subsec:bm_3}
The ultimate goal of addressing the \pb problem is to improve the success of long-horizon robot tasks. To this end, we introduce a challenge, \bmc, consisting of 10 long-horizon tasks\gb{again, it would be nice to list the tasks somewhere for completeness/reproducibility}, each comprising a chain of three skills (check examples in Figure~\ref{fig:bm_arch}). \bmc serves as a straightforward way to demonstrate the impact of the \pb problem on long-horizon task performance.

To construct \bmc, we manually select and combine skills from \taskoriginal \gb{I'm confused what's the difference between BOSS and BOSS-44}, ensuring that \pb occurs in each skill while avoiding conflicts between modifications. We reset the robot to a neutral position after each skill to eliminate dynamic transition feasibility issues~\cite{chen2023sequential}, ensuring the challenge focuses solely on the impact of \pb\gb{is that a realistic thing to do in real-world settings? Sounds contrived/artificial to me}. For \bmc, the sequential execution of multiple skill policies requires accounting for all their original performance, making it unsuitable to rely solely on PD\gb{What is PD? Use the full phrase so that the reader wouldn't have to find for acronym definition. I also don't understand what this sentence means}. Instead, we introduce a slightly different metric to evaluate the impact of accumulated \pb: \textbf{Delta to Upper Bound (DUB)}. DUB measures the difference between the success rate of completing the entire long-horizon task (i.e., achieving success for all skills in the chain) and an upper bound (UB). We compute the UB as the product of the success rates for each skill in the chain when evaluated without \pb, representing the maximum success rate achievable if \pb had no effect on long-horizon tasks. \gb{Again, I feel like the evaluation metric definitions should go under the experimental setup, not the benchmark description}




\subsection{Baselines}
\label{subsec:basic_bl}

\gb{To me this should also go under the experimental setup section along with the evaluation metrics}
% Overview
We select four widely used imitation learning algorithms, representing diverse architectures and design approaches for baseline comparisons, to learn each skill and evaluate the impact of \pb on their performance in long-horizon tasks.  Among these, three are Behavioral Cloning approaches, while one is a vision-language-action model.


% BC-RNN
% BC-Transformer
% BC-Vilt
\textbf{Behavioral Cloning (BC)}: A set of three BC algorithms~\cite{torabi2018behavioral} from Libero is adopted: BC-RESNET-RNN~\cite{mandlekar2021matters}, BC-RESNET-T~\cite{zhu2023viola}, and BC-VIT-T~\cite{kim2021vilt}. These algorithms feature diverse neural network architectures for visual and language encoding. All three use BERT embeddings~\cite{devlin2018bert} to encode the language instructions for each skill. In BC-RESNET-RNN, ResNet~\cite{he2016identity} serves as the visual backbone for encoding per-step visual observations, while an LSTM processes the sequence of encoded visual embeddings as the temporal backbone. BC-RESNET-T employs the same visual encoder, ResNet, but replaces the LSTM with a transformer decoder~\cite{vaswani2017attention} for temporal processing. BC-VIT-T uses Vision Transformer (ViT)~\cite{dosovitskiy2020image} as the visual backbone and a transformer decoder as the temporal backbone. All these BC algorithms output a multi-modal distribution over manipulation actions using a Gaussian Mixture Model (GMM) output head~\cite{bishop1994mixture}, from which an action is sampled.


% % Diffusion Policy
% \textbf{Diffusion Policy} --- Generative models have achieved remarkable success in language and vision domains~\cite{openai2024chatgpt, ramesh2022hierarchical, yang2024annotated}, making their application to robot learning a natural progression. Unlike Generative Adversarial Imitation Learning (GAIL)-like methods~\cite{ho2016generative}, which use Generative Adversarial Networks (GANs) as their backbone, diffusion policy~\cite{chi2023diffusion} achieves superior performance in robot learning due to its diffusion model backbone, offering multi-modal action distributions, handling high-dimensional outputs, and ensuring stable training. As a result, we select diffusion policy as the representative generative IL method to evaluate the impact of \pb problem.

% OpenVLA
\textbf{OpenVLA}: \yy{need to improve to include better motivation - need to relate to some motivations in the Introduction section?} Applying large foundation models, such as Large Language Models (LLMs)~\cite{openai2024chatgpt} and Vision-Language Models (VLMs)~\cite{dubey2024llama}, to robot learning has become a growing trend, culminating in the development of vision-language-action (VLA) models. These models leverage strong representation capabilities, task generalization, contextual understanding, and common sense reasoning to improve decision-making in robotics. Among these, OpenVLA~\cite{kim2024openvla}, an open-sourced VLA model, outperforms other state-of-the-art methods, making it our choice for evaluating the \pb problem as a representative generalist policy. \gb{I don't feel like you need such lengthy description for this. You can just say that given popularity of this method in recent years, you also adopt it to your evaluations as well.}


\subsection{Additional Baseline - Data Augmentation}
\label{subsec:our_bl}
% We propose a simple baseline, \bl, which additionally provides a corresponding dataset as a valuable byproduct. As defined in Section~\ref{sec:problem_definition}, the \pb problem arises when visual changes occur due to previous skills. A straightforward solution is to collect a larger set of demonstrations, allowing algorithms to learn from a diverse observation space and become robust to novel visual modifications. To explore the effectiveness of this potential solution to \pb, we augments demonstrations and train all the aforementioned baselines based on it to provide guidance for future research on the \pb problem. 
\gb{Subsection title is not very informative and just generally sounds weird. It also doesn't fit well with the benchmark section. Lastly, I think it hurts your paper to first introduce the benchmark and then suggest/imply that some simple approach can provide a solution to your benchmark. It defeats the purpose of your benchmark. I would formulate this as some additional baselines rather than the solution}

As defined in Section~\ref{sec:problem_definition}, the \pb problem arises when visual changes caused by previous skills disrupt current skill execution. A straightforward solution is to collect a larger and more diverse set of demonstrations, enabling algorithms to learn from varied observation spaces and become more robust to novel visual modifications. To evaluate the effectiveness of this approach, we augment the demonstrations and train all the aforementioned baselines on an expanded dataset.\gb{You can just call this Baselines with Data Augmentation or something like that. This is essentially just data augmentation. Not sure why we need to use vague terminology such as "potential solution" to a technique that's already widely used in other fields} %, offering valuable insights for future research on addressing the \pb problem. 

For each skill-level task, we scalably generate modified tasks with \pb problem using a \textbf{Rule-based Automatic Modification Generator (RAMG)}.\gb{To me the flow of this is not great, i.e., that you start talking about this 2 sections ago, don't conclude it, then have a separate completely unrelated subsection, and then go back to this again.} RAMG is a systematic algorithm designed to enhance diversity in pre-defined environments through structured, rule-based modifications. Operating on PDDL files, RAMG iteratively alters object positions, introduces new objects, or modifies object states within the environment. It supports three types of modifications: (1) repositioning or adding external objects to specific regions, (2) changing the states of fixtures (e.g., opening or closing cabinets), and (3) placing small objects into designated containers. These modifications follow dynamic constraints (e.g., newly added objects do not create obstacles) and maintain logical consistency (e.g., a drawer cannot be simultaneously open and closed) to ensure they do not hinder the agent from achieving the task goal. By utilizing deterministic yet flexible rules, RAMG offers a scalable approach to generating task variations, creating up to 1,727 modified tasks from the 44 tasks in \taskoriginal.

For each modified task generated by RAMG, we replay the demonstrations in the corresponding environment, creating new demonstrations where the trajectory remains the same but \pb is introduced. This approach produces a substantially larger demonstration dataset for each skill-level task. We then pre-train or fine-tune all the baselines using this augmented demonstration set to evaluate their performance when facing new \pb problem.\gb{What does it mean new OSS problem?}



==> sections/experiments.tex <==
\section{Experimental Results}
% Overview
\yy{I feel it not nice to include all results with table, suggestions for possible replacements (e.g., results figure) are needed}
In this section, we present results from experiments that seek to quantify and further understand \pb problem. We evaluate the baseline algorithms described in \S\ref{subsec:basic_bl} across the three benchmarks in \bm (Sections~\ref{subsec:results_bma}---\ref{subsec:results_bmc}) and conduct two experiments to identify the key factors contributing to the \pb problem (Section~\ref{subsec:factors}). Finally, we investigate whether data augmentation serves as an effective and straightforward solution to the \pb problem (Section~\ref{subsec:results_bl}).

\notezlf{I agree with the comments that the tables look overwhelming, maybe try to compress them / use figures, then you can move this to appendix (in extended version)}

\subsection{Results for \bma\gb{I find these weird names, i.e., Challenge 1, 2, 3. They are too generic and feel disconnected to the overall BOSS benchmark. Can we come up with something better?}}
\label{subsec:results_bma}
% 1. Use language to explain results
% 2. do some analyses

\input{tables/bm1_table}

We evaluate baseline methods, including BC-RESNET-RNN, BC-RESNET-T, BC-VIT-T, and OpenVLA, on the 44 original tasks and their 44 modified counterparts in \taskoriginal\gb{again, I'm confused about the difference between BOSS and BOSS-44}. As defined in Section~\ref{subsec:bm_1}, we use Performance Drop (PD) as the metric, calculated as the difference between the success rate on original tasks (SR-ORI) and the success rate on modified tasks (SR-MOD).\gb{Instead of repeating explanations about the evaluation metrics, just move them to the experiments section and create a separate paragraph/subsection for them} Table~\ref{tb:bm1_results} summarizes the average results across three random seeds, showing that \pb occurs in most tasks across all baselines. The ratios of positive PD\notezlf{I'd suggest to go to performance delta, then you can define positive+negative, and you don't really need to abbreviate here as it confuse people} (i.e., \pb occurrence) for BC-RESNET-RNN, BC-RESNET-T, BC-VIT-T, and OpenVLA are 68\%, 66\%, 50\%, and 66\%, respectively\gb{What is positive PD? It's very counterintuitive to put two words meaning opposite things, i.e., positive drop? What does that mean? I also can't relate to what you are saying to the things in the table as it's very overwhelming}. For tasks negatively affected by \pb, the average PD ratios are 29\%, 30\%, 28\%, and 44\%\gb{What are these ratios?}, respectively, underscoring the significant performance impact. These findings demonstrate that \pb frequently occurs even in single-step transitions, providing evidence that \pb can jeopardize the successful completion of long-horizon tasks. \gb{I feel like the definitions of you are evaluation metrics and the descriptions of these results + their connection to the table is not clear. I didn't understand much in this paragraph}



\subsection{Results for \bmb}
\label{subsec:results_bmb}

\input{tables/bm2_table}

As described in Section~\ref{subsec:bm_2}, we use the proposed RAMG to generate two sets of modified tasks: one with two modifications and another with three, simulating scenarios where \pb accumulates. Similar to \bma, we evaluate baselines on these modified tasks. Table~\ref{tb:bm2_results} presents average results across three random seeds alongside \bma outcomes (single-step modifications) for straightforward comparison. Due to space constraints, we report only the average success rate (Avg. SR) and average performance drop (Avg. PD). The results reveal that tasks with multiple modifications experience greater performance degradation (i.e., higher PD) compared to single-step modifications\gb{Can you provide concrete numbers to back this up?}. Furthermore, as the number of modifications increases, the negative impact becomes more pronounced, indicating that \pb accumulation significantly exacerbates task completion difficulty\gb{Again would be nice to present some numbers here}. Since \pb accumulation can occur frequently in long-horizon tasks, with the number of modifications growing along the skill chain, these findings further validate that \pb poses a significant challenge for long-horizon task completion.



\subsection{Results for \bmc}
\label{subsec:results_bmc}

\input{tables/bm3_table}

We include \bmc to evaluate the impact of \pb on real long-horizon tasks. As described in Section~\ref{subsec:bm_3}, we test baselines on 10 manually designed long-horizon tasks and introduce the DUB metric to quantify \pb's effect on task performance. Table~\ref{tb:bm3_results} presents average results across three random seeds, along with the Leveled Success Rate (Level SR), which measures success rates progressively along the skill chain: L0 represents the success rate for completing the first skill, L1 for completing the first two skills, and L2 for completing all three.\gb{I'm confused by this} The results indicate that DUB is positive and high in most cases, highlighting \pb's negative impact. The low DUB for BC-RESNET-RNN is attributed to its poor overall performance, resulting in a low UB. These findings from \bmc provide the clearest validation of the detrimental effect \pb has on long-horizon tasks. \gb{All the different evaluation metrics makes it difficult to understand these analyses. I didn't understand the main takeaways from these results}

\gb{Maybe instead of tables a bar plot would be a better way to present the results for all the challenges, especially if you want to include the results for all the tasks? I feel like tables are too overwhelming and don't look good in this case}



\subsection{Factors Influencing \pb}
\label{subsec:factors}

\input{tables/abl1_table}
\input{tables/abl2_table}

In this section, we examine two potential factors influencing the severity of \pb: task difficulty and the magnitude of visual modifications. This analysis aims to provide insights to guide future research and improve the development of algorithms robust to \pb. %robust IL algorithms.

\textbf{Task Difficulty:} We begin by investigating task difficulty as a factor. Task difficulty is quantified using task success rate, under the assumption that demonstrations provided for all tasks are of similar quality. To measure the severity of \pb, we introduce Relative Performance Drop (RPD) as a metric, defined as the PD divided by the original success rate. To isolate task difficulty as the sole changing factor and better analyze its relationship with \pb, we select six sets of tasks where all tasks in each set are performed within the same scene (e.g., kitchen scene 2 in Libero). For each set, we apply identical modifications to all tasks. Since the modifications introduced do not affect task feasibility, the hypothesis implies that when evaluating baselines on the tasks within a set, we should observe a higher RPD for tasks with lower success rates compared to those with higher success rates. After evaluation, for each set and each baseline, we obtain two lists of results: one for success rates on original tasks and another for PD on modified tasks. We use Spearman's rank correlation coefficient ($\rho$)~\cite{spearman1961proof} to test for a decreasing monotonic relationship between task success rate and RPD. Table~\ref{tb:fac1_results} summarizes the results for the baselines (excluding OpenVLA due to time constraints). In the table, $\rho$ indicates the Spearman correlation (a negative value implies a decreasing monotonic relationship), and $p$ represents the p-value. Ultimately, none of the baselines exhibited a significant decreasing monotonic relationship (i.e., $\rho < 0$, $p < 0.05$), and  thus we did not find evidence to support the hypothesis that task difficulty would be a key factor influencing the severity of \pb. \gb{I also find these results difficult to interpret from the Table. The table has a lot of numbers/details that are not clearly explained. Could this be better presented as some sort of plot? If not, then you need to simplify the table. I also feel like this analysis is convoluted/overhwelming. In my view, it's possible to summarize the main findings in a much simpler way, and also more concisely.}

\textbf{Magnitude of Visual Modification:} The magnitude of visual modification is another factor that may influence the severity of \pb. We use PD as a metric to explore this potential relationship. To ensure that the magnitude of visual modification is the only variable changing, we follow a similar approach to \bmb by increasing the number of modifications applied to the same task. Unlike the random RAMG-generated modifications used in \bmb, we incrementally add new modifications based on existing ones, ensuring a clear correlation between the number of modifications and the size of the visual changes. Our hypothesis is that increasing the magnitude of visual modifications (i.e., the number of modifications) will result in a greater negative effect (i.e., higher PD) caused by \pb. We test this hypothesis using three baselines evaluated on 10 tasks for each modification level. Due to space constraints, Table~\ref{tb:fac2_results} presents the average results, which show that PD consistently increases for each baseline as the magnitude of visual modifications grows. These findings support the hypothesis that the magnitude of visual modifications may be a key factor influencing the severity of \pb.\gb{I'm a bit confused by this experiment. Are you showing something different here than you did for Challenge 2 where you also studied PD as a function of modifications? Also, your table for this is extremely uninformative. It's not clear what the values in the table actually measure. The table doesn't have any useful captions. If I just looked at the table, I would have no idea what I'm looking at.}

\subsection{Data Augmentation for \pb}
\label{subsec:results_bl}

\input{tables/da_table}

% intro the dataset we use for training
% intro the confusion matrix
% 1. pd is small
% 2. C - D is bad <= cuased by B's drop (even for OpenVLA)
% conclusion: it's not that straightforward to directly use data augmentation way to solve the \pb issue. Need special design.

% As stated in Section~\ref{subsec:our_bl}, we pre-train or finetune baselines on the large dataset generated via RAMG. To identify the effect of the simple data augmentation method, we compare the following 4 types of results:
% \begin{enumerate}[A.]
%     \item Trained on demonstrations of single environment-1, Evaluated on the same environment-1.
%     \item Trained on augmented mixtured demonstrations of diverse environment, Evaluated on the environment-1.
%     \item Trained on demonstrations of single environment-1, Evaluated on the modified environment-1.
%     \item Trained on augmented mixtured demonstrations of diverse environment, Evaluated on the modified environment-1.
% \end{enumerate}

% Table~\ref{tb:da_results} shows the above 4 types of results for baselines. When trained with augmented mistured demonstrations, although we could observe nearly 0 PD for all 3 BCs by comparing results-B and results-D, this does not prove that using more diverse training demonstrations could largely mitigate \pb problem. When comparing results-C and results-D where the baselines are both evaluated on modified environment but one (C) is trained only with original environment demonstration and the other one (D) is trained with augmented mixtured data, we could see that only BC-RESNET-RNN shows a bit improvement, and the other three baselines all present equivalent or even worse performance. By comparing results-A and results-B where baselines are both evaluated on the seen environment, we could find out that the current IL baselines, even for OpenVLA which is the generalist policy, will face performance drop when trained on larger and more diverse dataset. Therefore, we could conclude that simply trained on more diverse and larger dataset cannot bring clear improvement, the \pb problem is a severe problem that need some specific method design.



As described in Section~\ref{subsec:our_bl}, we pre-train or fine-tune baselines on the large and much more visual diverse dataset generated using RAMG. To analyze the impact of the data augmentation method, we compare the following four experimental setups, all designed for the same task but differing in the visual characteristics of the training and evaluation environments:
\begin{enumerate}[A.] 
    \item Trained on single-environment, noted as Env-X, demonstrations and evaluated on the same environment (i.e., Env-X). 
    \item Trained on augmented demonstrations from diverse environments and evaluated on Env-X. 
    \item Trained on Env-X and evaluated on the modified version of Env-X. 
    \item Trained on augmented demonstrations from diverse environments and evaluated on the modified version of Env-X. 
\end{enumerate} 
\gb{I understand these four settings but this is too complex and most readers will be lost/overwhelmed by these setups. You need to find a way to present these in a simpler manner}

Table~\ref{tb:da_results} presents average results across three random seeds for these setups across all baselines, with only the averaged results across all 44 tasks reported due to space constraints. Several key observations emerge from the results. Comparing Results-C and Results-D, where baselines are evaluated on the modified environment, shows that BC-RESNET-RNN exhibits slight improvement in D. However, other baselines, including BC-RESNET-T, BC-VIT-T, and OpenVLA, perform equivalently or worse, highlighting the limited effectiveness of data augmentation in mitigating \pb. A possible explanation emerges from comparing Results-A and Results-B, where baselines are evaluated on the same original environment. This comparison shows that training on a larger but more diverse dataset leads to performance drops across all baselines, including OpenVLA, the generalist policy. These findings indicate that simply training on larger and more diverse datasets is insufficient to address \pb effectively, emphasizing the need for specific algorithmic solutions.\gb{Do we really need baselines A and B? What do they contribute to this analysis? Generally, for me it was difficult to follow this analysis as well. }

==> tables/abl2_table.tex <==
\begin{table}[]
\centering
\caption{Results on the relationship between visual modification size and OSS severity.}
\label{tb:fac2_results}
\begin{tabular}{|c|c|c|c|}
\hline
                                                                 & BC-RESNET-RNN & BC-RESNET-T & BC-VIT-T \\ \hline
\begin{tabular}[c]{@{}c@{}}PD\\ (1 modification)\end{tabular} & 0.13          & 0.06        & 0.10     \\ \hline
\begin{tabular}[c]{@{}c@{}}PD\\ (2 modification)\end{tabular} & 0.25          & 0.24        & 0.13     \\ \hline
\begin{tabular}[c]{@{}c@{}}PD\\ (3 modification)\end{tabular} & 0.77          & 0.77        & 0.34     \\ \hline
\end{tabular}
\end{table}


==> tables/bm1_table.tex <==
        % Please add the following required packages to your document preamble:
        % \usepackage{multirow}
        % \usepackage{xcolor}
        
        \begin{table*}[!htb]
        \scriptsize
        \setlength{\tabcolsep}{2pt} % Adjust the margin between columns
        \renewcommand{\arraystretch}{1.1} % Adjust the row height
        \centering
        \caption{Challenge-1 results, evaluating 4 IL methods on tasks in \taskoriginal, highlighting those with positive performance drops.}
        \label{tb:bm1_results}
        \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
        \hline
                                   &          & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 \\ \hline

\multirow{3}{*}{BC-RESNET-RNN} & SR - ORI & 0.98 & 0.73 & 0.78 & 0.97 & 0.00 & 0.02 & 0.63 & 0.05 & 0.15 & 0.00 & 0.07 & 0.63 & 0.00 & 0.52 & 0.40 & 1.00 & 0.98 & 0.00 & 0.27 & 0.25 & 0.63 & 0.52 \\ \cline{2-24}
                                    & SR - MOD & 1.00 & 0.20 & 0.65 & 0.32 & 0.02 & 0.00 & 0.00 & 0.02 & 0.07 & 0.00 & 0.08 & 0.23 & 0.00 & 0.60 & 0.10 & 0.37 & 0.43 & 0.00 & 0.37 & 0.27 & 0.52 & 0.32 \\ \cline{2-24}
                                    & PD    & -0.02 & \textbf{\textcolor{red}{0.53}} & \textbf{\textcolor{red}{0.13}} & \textbf{\textcolor{red}{0.65}} & -0.02 & \textbf{\textcolor{red}{0.02}} & \textbf{\textcolor{red}{0.63}} & \textbf{\textcolor{red}{0.03}} & \textbf{\textcolor{red}{0.08}} & 0.00 & -0.02 & \textbf{\textcolor{red}{0.40}} & 0.00 & -0.08 & \textbf{\textcolor{red}{0.30}} & \textbf{\textcolor{red}{0.63}} & \textbf{\textcolor{red}{0.55}} & 0.00 & -0.10 & -0.02 & \textbf{\textcolor{red}{0.12}} & \textbf{\textcolor{red}{0.20}} \\ \hline

        \multirow{3}{*}{BC-RESNET-T} & SR - ORI & 1.00 & 1.00 & 1.00 & 0.95 & 0.93 & 1.00 & 0.95 & 0.83 & 0.82 & 0.63 & 0.97 & 0.92 & 0.42 & 1.00 & 0.87 & 1.00 & 0.98 & 0.90 & 0.92 & 0.73 & 0.73 & 1.00 \\ \cline{2-24}
                                    & SR - MOD & 1.00 & 0.67 & 0.93 & 0.12 & 0.82 & 0.22 & 0.98 & 0.62 & 0.17 & 0.62 & 1.00 & 0.53 & 0.52 & 0.87 & 0.57 & 1.00 & 0.93 & 0.12 & 0.63 & 0.78 & 0.58 & 0.97 \\ \cline{2-24}
                                    & PD    & 0.00 & \textbf{\textcolor{red}{0.33}} & \textbf{\textcolor{red}{0.07}} & \textbf{\textcolor{red}{0.83}} & \textbf{\textcolor{red}{0.12}} & \textbf{\textcolor{red}{0.78}} & -0.03 & \textbf{\textcolor{red}{0.22}} & \textbf{\textcolor{red}{0.65}} & \textbf{\textcolor{red}{0.02}} & -0.03 & \textbf{\textcolor{red}{0.38}} & -0.10 & \textbf{\textcolor{red}{0.13}} & \textbf{\textcolor{red}{0.30}} & 0.00 & \textbf{\textcolor{red}{0.05}} & \textbf{\textcolor{red}{0.78}} & \textbf{\textcolor{red}{0.28}} & -0.05 & \textbf{\textcolor{red}{0.15}} & \textbf{\textcolor{red}{0.03}} \\ \hline
\multirow{3}{*}{BC-VIT-T} & SR - ORI & 1.00 & 1.00 & 0.98 & 0.95 & 0.95 & 0.98 & 0.98 & 0.87 & 0.68 & 0.55 & 0.98 & 0.90 & 0.92 & 0.90 & 0.98 & 1.00 & 1.00 & 0.98 & 0.98 & 0.70 & 0.63 & 1.00 \\ \cline{2-24}
                                    & SR - MOD & 1.00 & 0.65 & 1.00 & 0.97 & 0.82 & 0.13 & 0.97 & 0.92 & 0.30 & 0.68 & 0.73 & 0.28 & 0.88 & 0.68 & 0.77 & 1.00 & 1.00 & 0.00 & 0.73 & 0.63 & 0.67 & 1.00 \\ \cline{2-24}
                                    & PD    & 0.00 & \textbf{\textcolor{red}{0.35}} & -0.02 & -0.02 & \textbf{\textcolor{red}{0.13}} & \textbf{\textcolor{red}{0.85}} & \textbf{\textcolor{red}{0.02}} & -0.05 & \textbf{\textcolor{red}{0.38}} & -0.13 & \textbf{\textcolor{red}{0.25}} & \textbf{\textcolor{red}{0.62}} & \textbf{\textcolor{red}{0.03}} & \textbf{\textcolor{red}{0.22}} & \textbf{\textcolor{red}{0.22}} & 0.00 & 0.00 & \textbf{\textcolor{red}{0.98}} & \textbf{\textcolor{red}{0.25}} & \textbf{\textcolor{red}{0.07}} & -0.03 & 0.00 \\ \hline
\multirow{3}{*}{OpenVLA} & SR - ORI & 1.00 & 1.00 & 0.65 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.70 & 0.65 & 0.65 & 0.50 & 0.75 & 0.80 & 1.00 & 0.85 & 0.80 & 0.95 & 0.40 & 1.00 \\ \cline{2-24}
                                    & SR - MOD & 0.35 & 1.00 & 0.55 & 0.00 & 1.00 & 0.70 & 0.00 & 1.00 & 0.30 & 0.65 & 0.35 & 1.00 & 1.00 & 0.55 & 0.75 & 0.20 & 0.75 & 0.05 & 0.55 & 0.35 & 0.15 & 1.00 \\ \cline{2-24}
                                    & PD    & \textbf{\textcolor{red}{0.65}} & 0.00 & \textbf{\textcolor{red}{0.10}} & \textbf{\textcolor{red}{1.00}} & 0.00 & \textbf{\textcolor{red}{0.30}} & \textbf{\textcolor{red}{1.00}} & 0.00 & \textbf{\textcolor{red}{0.70}} & \textbf{\textcolor{red}{0.35}} & \textbf{\textcolor{red}{0.35}} & -0.35 & -0.35 & -0.05 & 0.00 & \textbf{\textcolor{red}{0.60}} & \textbf{\textcolor{red}{0.25}} & \textbf{\textcolor{red}{0.80}} & \textbf{\textcolor{red}{0.25}} & \textbf{\textcolor{red}{0.60}} & \textbf{\textcolor{red}{0.25}} & 0.00 \\ \hline
% \multirow{3}{*}{MaIL} & SR - ORI & 0.93 & 1.00 & 0.43 & 0.93 & 0.93 & 0.97 & 0.95 & 0.70 & 0.73 & 0.90 & 0.52 & 0.52 & 0.28 & 0.95 & 0.35 & 1.00 & 0.97 & 0.92 & 1.00 & 0.20 & 0.18 & 0.98 \\ \cline{2-24}
%                                     & SR - MOD & 0.95 & 0.00 & 0.58 & 0.00 & 0.00 & 0.15 & 0.00 & 0.57 & 0.28 & 0.83 & 0.92 & 0.42 & 0.13 & 0.60 & 0.00 & 0.45 & 0.83 & 0.00 & 0.92 & 0.27 & 0.37 & 0.93 \\ \cline{2-24}
%                                     & PD    & -0.02 & \textbf{\textcolor{red}{1.00}} & -0.15 & \textbf{\textcolor{red}{0.93}} & \textbf{\textcolor{red}{0.93}} & \textbf{\textcolor{red}{0.82}} & \textbf{\textcolor{red}{0.95}} & \textbf{\textcolor{red}{0.13}} & \textbf{\textcolor{red}{0.45}} & \textbf{\textcolor{red}{0.07}} & -0.40 & \textbf{\textcolor{red}{0.10}} & \textbf{\textcolor{red}{0.15}} & \textbf{\textcolor{red}{0.35}} & \textbf{\textcolor{red}{0.35}} & \textbf{\textcolor{red}{0.55}} & \textbf{\textcolor{red}{0.13}} & \textbf{\textcolor{red}{0.92}} & \textbf{\textcolor{red}{0.08}} & -0.07 & -0.18 & \textbf{\textcolor{red}{0.05}} \\ \hline

        \end{tabular}
        \end{table*}
        
        % Please add the following required packages to your document preamble:
        % \usepackage{multirow}
        % \usepackage{xcolor}




        \vspace{-30em}
        \begin{table*}[!htb]
        \scriptsize
        \setlength{\tabcolsep}{2pt} % Adjust the margin between columns
        \renewcommand{\arraystretch}{1.1} % Adjust the row height
        \centering
        \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
        \hline
                                   &          & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 \\ \hline

\multirow{3}{*}{BC-RESNET-RNN} & SR - ORI & 0.87 & 0.00 & 0.03 & 0.15 & 0.33 & 1.00 & 0.65 & 0.45 & 0.58 & 0.85 & 0.75 & 0.18 & 0.92 & 0.73 & 1.00 & 0.00 & 0.02 & 0.15 & 0.08 & 0.07 & 0.12 & 0.45 \\ \cline{2-24}
                                    & SR - MOD & 0.72 & 0.02 & 0.00 & 0.07 & 0.52 & 0.95 & 0.40 & 0.07 & 0.65 & 0.23 & 0.35 & 0.00 & 0.63 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.03 \\ \cline{2-24}
                                    & PD    & \textbf{\textcolor{red}{0.15}} & -0.02 & \textbf{\textcolor{red}{0.03}} & \textbf{\textcolor{red}{0.08}} & -0.18 & \textbf{\textcolor{red}{0.05}} & \textbf{\textcolor{red}{0.25}} & \textbf{\textcolor{red}{0.38}} & -0.07 & \textbf{\textcolor{red}{0.62}} & \textbf{\textcolor{red}{0.40}} & \textbf{\textcolor{red}{0.18}} & \textbf{\textcolor{red}{0.28}} & \textbf{\textcolor{red}{0.73}} & 0.00 & 0.00 & \textbf{\textcolor{red}{0.02}} & \textbf{\textcolor{red}{0.15}} & \textbf{\textcolor{red}{0.08}} & \textbf{\textcolor{red}{0.05}} & \textbf{\textcolor{red}{0.12}} & \textbf{\textcolor{red}{0.42}} \\ \hline

        \multirow{3}{*}{BC-RESNET-T} & SR - ORI & 1.00 & 0.27 & 0.98 & 0.47 & 0.97 & 1.00 & 0.65 & 0.57 & 1.00 & 0.98 & 0.93 & 0.98 & 0.95 & 0.85 & 1.00 & 0.47 & 0.65 & 0.60 & 0.48 & 0.90 & 0.70 & 0.53 \\ \cline{2-24}
                                    & SR - MOD & 0.97 & 0.33 & 0.95 & 0.60 & 0.90 & 1.00 & 0.38 & 0.80 & 0.90 & 0.42 & 0.75 & 0.88 & 0.98 & 0.07 & 1.00 & 0.52 & 1.00 & 0.78 & 0.00 & 0.90 & 0.30 & 0.30 \\ \cline{2-24}
                                    & PD    & \textbf{\textcolor{red}{0.03}} & -0.07 & \textbf{\textcolor{red}{0.03}} & -0.13 & \textbf{\textcolor{red}{0.07}} & 0.00 & \textbf{\textcolor{red}{0.27}} & -0.23 & \textbf{\textcolor{red}{0.10}} & \textbf{\textcolor{red}{0.57}} & \textbf{\textcolor{red}{0.18}} & \textbf{\textcolor{red}{0.10}} & -0.03 & \textbf{\textcolor{red}{0.78}} & 0.00 & -0.05 & -0.35 & -0.18 & \textbf{\textcolor{red}{0.48}} & 0.00 & \textbf{\textcolor{red}{0.40}} & \textbf{\textcolor{red}{0.23}} \\ \hline
\multirow{3}{*}{BC-VIT-T} & SR - ORI & 0.98 & 0.50 & 0.93 & 0.48 & 0.95 & 0.98 & 0.82 & 0.72 & 0.98 & 1.00 & 0.65 & 0.95 & 0.85 & 0.95 & 1.00 & 0.38 & 0.80 & 0.72 & 0.37 & 0.77 & 0.65 & 0.57 \\ \cline{2-24}
                                    & SR - MOD & 1.00 & 0.33 & 1.00 & 0.62 & 0.93 & 1.00 & 0.30 & 0.57 & 0.95 & 0.72 & 0.87 & 0.85 & 0.87 & 0.83 & 1.00 & 0.67 & 0.82 & 0.77 & 0.00 & 0.77 & 0.88 & 0.87 \\ \cline{2-24}
                                    & PD    & -0.02 & \textbf{\textcolor{red}{0.17}} & -0.07 & -0.13 & \textbf{\textcolor{red}{0.02}} & -0.02 & \textbf{\textcolor{red}{0.52}} & \textbf{\textcolor{red}{0.15}} & \textbf{\textcolor{red}{0.03}} & \textbf{\textcolor{red}{0.28}} & -0.22 & \textbf{\textcolor{red}{0.10}} & -0.02 & \textbf{\textcolor{red}{0.12}} & 0.00 & -0.28 & -0.02 & -0.05 & \textbf{\textcolor{red}{0.37}} & 0.00 & -0.23 & -0.30 \\ \hline
\multirow{3}{*}{OpenVLA} & SR - ORI & 1.00 & 0.90 & 1.00 & 0.45 & 0.95 & 1.00 & 0.65 & 0.95 & 0.75 & 0.40 & 0.60 & 0.95 & 0.85 & 0.85 & 0.90 & 1.00 & 0.35 & 1.00 & 0.00 & 1.00 & 0.70 & 0.65 \\ \cline{2-24}
                                    & SR - MOD & 1.00 & 0.55 & 0.65 & 0.35 & 0.85 & 1.00 & 0.70 & 0.65 & 0.15 & 0.05 & 0.50 & 0.60 & 0.80 & 0.95 & 0.00 & 0.65 & 0.35 & 0.30 & 0.00 & 0.30 & 1.00 & 0.00 \\ \cline{2-24}
                                    & PD    & 0.00 & \textbf{\textcolor{red}{0.35}} & \textbf{\textcolor{red}{0.35}} & \textbf{\textcolor{red}{0.10}} & \textbf{\textcolor{red}{0.10}} & 0.00 & -0.05 & \textbf{\textcolor{red}{0.30}} & \textbf{\textcolor{red}{0.60}} & \textbf{\textcolor{red}{0.35}} & \textbf{\textcolor{red}{0.10}} & \textbf{\textcolor{red}{0.35}} & \textbf{\textcolor{red}{0.05}} & -0.10 & \textbf{\textcolor{red}{0.90}} & \textbf{\textcolor{red}{0.35}} & 0.00 & \textbf{\textcolor{red}{0.70}} & 0.00 & \textbf{\textcolor{red}{0.70}} & -0.30 & \textbf{\textcolor{red}{0.65}} \\ \hline
% \multirow{3}{*}{MaIL} & SR - ORI & 0.98 & 0.82 & 0.93 & 0.27 & 0.38 & 0.68 & 0.80 & 0.90 & 0.55 & 0.85 & 0.25 & 0.97 & 0.18 & 0.95 & 1.00 & 0.57 & 0.85 & 0.62 & 0.93 & 0.53 & 0.93 & 0.10 \\ \cline{2-24}
%                                     & SR - MOD & 0.97 & 0.20 & 0.92 & 0.55 & 0.17 & 0.07 & 0.55 & 0.42 & 0.02 & 0.73 & 0.27 & 0.93 & 0.77 & 0.35 & 0.53 & 0.58 & 0.33 & 0.38 & 0.00 & 0.53 & 0.20 & 0.17 \\ \cline{2-24}
%                                     & PD    & \textbf{\textcolor{red}{0.02}} & \textbf{\textcolor{red}{0.62}} & \textbf{\textcolor{red}{0.02}} & -0.28 & \textbf{\textcolor{red}{0.22}} & \textbf{\textcolor{red}{0.62}} & \textbf{\textcolor{red}{0.25}} & \textbf{\textcolor{red}{0.48}} & \textbf{\textcolor{red}{0.53}} & \textbf{\textcolor{red}{0.12}} & -0.02 & \textbf{\textcolor{red}{0.03}} & -0.58 & \textbf{\textcolor{red}{0.60}} & \textbf{\textcolor{red}{0.47}} & -0.02 & \textbf{\textcolor{red}{0.52}} & \textbf{\textcolor{red}{0.23}} & \textbf{\textcolor{red}{0.93}} & 0.00 & \textbf{\textcolor{red}{0.73}} & -0.07 \\ \hline

        \end{tabular}
        \end{table*}
        

==> tables/bm2_table.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \caption{Results for BM2}
% \label{tb:bm2_results}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
%                                  &                              & BC-RESNET-RNN & BC-RESNET-T & BC-VIT-T & OpenVLA & MaIL                      \\ \hline
% \multicolumn{1}{|l|}{Original}   & \multicolumn{1}{l|}{Avg. SR} & 0.43          & 0.83        & 0.84     & 0.81    & \multicolumn{1}{l|}{0.71} \\ \hline
% \multirow{2}{*}{1 Modification}  & Avg. SR                      & 0.25          & 0.67        & 0.74     & 0.54    & 0.43                      \\ \cline{2-7} 
%                                  & Avg. PD                        & 0.18          & 0.16        & 0.10     & 0.27    & 0.28                      \\ \hline
% \multirow{2}{*}{2 Modifications} & Avg. SR                      & 0.25          & 0.55        & 0.53     & 0.46    &                           \\ \cline{2-7} 
%                                  & Avg. PD                        & 0.18          & 0.28        & 0.31     & 0.35    &                           \\ \hline
% \multirow{2}{*}{3 Modifications} & Avg. SR                      & 0.23          & 0.49        & 0.56     & 0.35    &                           \\ \cline{2-7} 
%                                  & Avg. PD                        & 0.20          & 0.34        & 0.28     & 0.46    &                           \\ \hline
% \end{tabular}
% \end{table*}






% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Challenge-2 results, evaluating four IL methods on \taskoriginal, with averages shown across tasks.}
\label{tb:bm2_results}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
                                 &                              & BC-RESNET-RNN & BC-RESNET-T & BC-VIT-T & OpenVLA \\ \hline
\multicolumn{1}{|l|}{Original}   & \multicolumn{1}{l|}{Avg. SR} & 0.43          & 0.83        & 0.84     & 0.81    \\ \hline
\multirow{2}{*}{1 Modification}  & Avg. SR                      & 0.25          & 0.67        & 0.74     & 0.54    \\ \cline{2-6} 
                                 & Avg. PD                      & 0.18          & 0.16        & 0.10     & 0.27    \\ \hline
\multirow{2}{*}{2 Modifications} & Avg. SR                      & 0.25          & 0.55        & 0.53     & 0.46    \\ \cline{2-6} 
                                 & Avg. PD                      & 0.18          & 0.28        & 0.31     & 0.35    \\ \hline
\multirow{2}{*}{3 Modifications} & Avg. SR                      & 0.23          & 0.49        & 0.56     & 0.35    \\ \cline{2-6} 
                                 & Avg. PD                      & 0.20          & 0.34        & 0.28     & 0.46    \\ \hline
\end{tabular}
\end{table*}


==> tables/bm3_table.tex <==
% \begin{table*}[]
% \scriptsize
% \centering
% \caption{Results for BM3}
% \label{tb:bm3_results}
% \begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|}
% \hline
%    & \multicolumn{3}{c|}{BC-RESNET-RNN}                                                   & \multicolumn{3}{c|}{BC-RESNET-T}                                                     & \multicolumn{3}{c|}{BC-VIT-T}                                                        & \multicolumn{3}{c|}{OpenVLA}                                                           & \multicolumn{3}{c|}{MaIL}                                     \\ \hline
%    & \multicolumn{1}{c|}{Level SR}                     & \multicolumn{1}{c|}{UB}   & DUB  & \multicolumn{1}{c|}{Level SR}                     & \multicolumn{1}{c|}{UB}   & DUB  & \multicolumn{1}{c|}{Level SR}                     & \multicolumn{1}{c|}{UB}   & DUB  & \multicolumn{1}{c|}{Level SR}                      & \multicolumn{1}{c|}{UB}   & DUB   & \multicolumn{1}{c|}{Level SR} & \multicolumn{1}{c|}{UB} & DUB \\ \hline
% 1  & \multicolumn{1}{c|}{\makecell{L0: 0.85 \\ L1: 0.3 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.01} & 0.01 & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.1 \\ L2: 0.1}}  & \multicolumn{1}{c|}{0.95} & 0.85 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 1.0 \\ L2: 0.2}}   & \multicolumn{1}{c|}{0.92} & 0.72 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.0 \\ L2: 0.0}}    & \multicolumn{1}{c|}{0.65} & 0.65  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 2  & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.0 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.01} & 0.01 & \multicolumn{1}{c|}{\makecell{L0: 0.9 \\ L1: 0.15 \\ L2: 0.05}} & \multicolumn{1}{c|}{0.95} & 0.90 & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.25 \\ L2: 0.1}} & \multicolumn{1}{c|}{0.92} & 0.82 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.0 \\ L2: 0.0}}    & \multicolumn{1}{c|}{1.00} & 1.00  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 3  & \multicolumn{1}{c|}{\makecell{L0: 0.55 \\ L1: 0.0 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.00} & 0.00 & \multicolumn{1}{c|}{\makecell{L0: 0.9 \\ L1: 0.0 \\ L2: 0.0}}   & \multicolumn{1}{c|}{0.77} & 0.77 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.1 \\ L2: 0.1}}   & \multicolumn{1}{c|}{0.84} & 0.74 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.15 \\ L2: 0.05}}  & \multicolumn{1}{c|}{0.70} & 0.65  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 4  & \multicolumn{1}{c|}{\makecell{L0: 0.4 \\ L1: 0.05 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.01} & 0.01 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.7 \\ L2: 0.2}}   & \multicolumn{1}{c|}{0.75} & 0.55 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.75 \\ L2: 0.65}} & \multicolumn{1}{c|}{0.66} & 0.01 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.75 \\ L2: 0.65}}  & \multicolumn{1}{c|}{0.70} & 0.05  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 5  & \multicolumn{1}{c|}{\makecell{L0: 0.4 \\ L1: 0.0 \\ L2: 0.0}}   & \multicolumn{1}{c|}{0.07} & 0.07 & \multicolumn{1}{c|}{\makecell{L0: 0.6 \\ L1: 0.25 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.66} & 0.66 & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.65 \\ L2: 0.6}}  & \multicolumn{1}{c|}{0.69} & 0.09 & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.65 \\ L2: 0.35}}  & \multicolumn{1}{c|}{0.76} & 0.41  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 6  & \multicolumn{1}{c|}{\makecell{L0: 0.45 \\ L1: 0.2 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.07} & 0.07 & \multicolumn{1}{c|}{\makecell{L0: 0.75 \\ L1: 0.5 \\ L2: 0.1}}  & \multicolumn{1}{c|}{0.66} & 0.56 & \multicolumn{1}{c|}{\makecell{L0: 0.75 \\ L1: 0.65 \\ L2: 0.3}} & \multicolumn{1}{c|}{0.69} & 0.39 & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.35 \\ L2: 0.1}}   & \multicolumn{1}{c|}{0.76} & 0.66  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 7  & \multicolumn{1}{c|}{\makecell{L0: 0.0 \\ L1: 0.0 \\ L2: 0.0}}   & \multicolumn{1}{c|}{0.00} & 0.00 & \multicolumn{1}{c|}{\makecell{L0: 0.85 \\ L1: 0.85 \\ L2: 0.3}} & \multicolumn{1}{c|}{0.65} & 0.35 & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.65 \\ L2: 0.4}} & \multicolumn{1}{c|}{0.62} & 0.22 & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.65 \\ L2: 0.15}} & \multicolumn{1}{c|}{0.34} & 0.19  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 8  & \multicolumn{1}{c|}{\makecell{L0: 0.4 \\ L1: 0.0 \\ L2: 0.0}}   & \multicolumn{1}{c|}{0.00} & 0.00 & \multicolumn{1}{c|}{\makecell{L0: 0.65 \\ L1: 0.4 \\ L2: 0.35}} & \multicolumn{1}{c|}{0.65} & 0.30 & \multicolumn{1}{c|}{\makecell{L0: 0.7 \\ L1: 0.7 \\ L2: 0.5}}   & \multicolumn{1}{c|}{0.62} & 0.12 & \multicolumn{1}{c|}{\makecell{L0: 0.5 \\ L1: 0.25 \\ L2: 0.2}}   & \multicolumn{1}{c|}{0.34} & 0.14  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 9  & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.05 \\ L2: 0.05}} & \multicolumn{1}{c|}{0.55} & 0.50 & \multicolumn{1}{c|}{\makecell{L0: 0.9 \\ L1: 0.2 \\ L2: 0.2}}   & \multicolumn{1}{c|}{0.79} & 0.59 & \multicolumn{1}{c|}{\makecell{L0: 0.7 \\ L1: 0.5 \\ L2: 0.5}}   & \multicolumn{1}{c|}{0.62} & 0.12 & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.7 \\ L2: 0.7}}    & \multicolumn{1}{c|}{0.46} & -0.24 & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% 10 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.1 \\ L2: 0.1}}   & \multicolumn{1}{c|}{0.67} & 0.57 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.45 \\ L2: 0.45}} & \multicolumn{1}{c|}{0.81} & 0.36 & \multicolumn{1}{c|}{\makecell{L0: 0.85 \\ L1: 0.6 \\ L2: 0.6}}  & \multicolumn{1}{c|}{0.81} & 0.21 & \multicolumn{1}{c|}{\makecell{L0: 0.9 \\ L1: 0.55 \\ L2: 0.55}}  & \multicolumn{1}{c|}{0.65} & 0.10  & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}   &     \\ \hline
% \end{tabular}
% \end{table*}


\begin{table*}[ht]
\scriptsize
\centering
\caption{Challenge-3 results, evaluating four IL methods on \taskoriginal, with averages shown across tasks.}
\label{tb:bm3_results}
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
   & \multicolumn{3}{c|}{BC-RESNET-RNN}                                                   & \multicolumn{3}{c|}{BC-RESNET-T}                                                     & \multicolumn{3}{c|}{BC-VIT-T}                                                        & \multicolumn{3}{c}{OpenVLA}                                                           \\ \midrule
   & \multicolumn{1}{c|}{Level SR}                     & \multicolumn{1}{c|}{UB}   & DUB  & \multicolumn{1}{c|}{Level SR}                     & \multicolumn{1}{c|}{UB}   & DUB  & \multicolumn{1}{c|}{Level SR}                     & \multicolumn{1}{c|}{UB}   & DUB  & \multicolumn{1}{c|}{Level SR}                      & \multicolumn{1}{c|}{UB}   & DUB   \\ \midrule
1  & \multicolumn{1}{c|}{\makecell{L0: 0.85 \\ L1: 0.3 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.01} & 0.01 & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.1 \\ L2: 0.1}}  & \multicolumn{1}{c|}{0.95} & 0.85 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 1.0 \\ L2: 0.2}}   & \multicolumn{1}{c|}{0.92} & 0.72 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.0 \\ L2: 0.0}}    & \multicolumn{1}{c|}{0.65} & 0.65  \\ \midrule
2  & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.0 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.01} & 0.01 & \multicolumn{1}{c|}{\makecell{L0: 0.9 \\ L1: 0.15 \\ L2: 0.05}} & \multicolumn{1}{c|}{0.95} & 0.90 & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.25 \\ L2: 0.1}} & \multicolumn{1}{c|}{0.92} & 0.82 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.0 \\ L2: 0.0}}    & \multicolumn{1}{c|}{1.00} & 1.00  \\ \midrule
3  & \multicolumn{1}{c|}{\makecell{L0: 0.55 \\ L1: 0.0 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.00} & 0.00 & \multicolumn{1}{c|}{\makecell{L0: 0.9 \\ L1: 0.0 \\ L2: 0.0}}   & \multicolumn{1}{c|}{0.77} & 0.77 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.1 \\ L2: 0.1}}   & \multicolumn{1}{c|}{0.84} & 0.74 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.15 \\ L2: 0.05}}  & \multicolumn{1}{c|}{0.70} & 0.65  \\ \midrule
4  & \multicolumn{1}{c|}{\makecell{L0: 0.4 \\ L1: 0.05 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.01} & 0.01 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.7 \\ L2: 0.2}}   & \multicolumn{1}{c|}{0.75} & 0.55 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.75 \\ L2: 0.65}} & \multicolumn{1}{c|}{0.66} & 0.01 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.75 \\ L2: 0.65}}  & \multicolumn{1}{c|}{0.70} & 0.05  \\ \midrule
5  & \multicolumn{1}{c|}{\makecell{L0: 0.4 \\ L1: 0.0 \\ L2: 0.0}}   & \multicolumn{1}{c|}{0.07} & 0.07 & \multicolumn{1}{c|}{\makecell{L0: 0.6 \\ L1: 0.25 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.66} & 0.66 & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.65 \\ L2: 0.6}}  & \multicolumn{1}{c|}{0.69} & 0.09 & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.65 \\ L2: 0.35}}  & \multicolumn{1}{c|}{0.76} & 0.41  \\ \midrule
6  & \multicolumn{1}{c|}{\makecell{L0: 0.45 \\ L1: 0.2 \\ L2: 0.0}}  & \multicolumn{1}{c|}{0.07} & 0.07 & \multicolumn{1}{c|}{\makecell{L0: 0.75 \\ L1: 0.5 \\ L2: 0.1}}  & \multicolumn{1}{c|}{0.66} & 0.56 & \multicolumn{1}{c|}{\makecell{L0: 0.75 \\ L1: 0.65 \\ L2: 0.3}} & \multicolumn{1}{c|}{0.69} & 0.39 & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.35 \\ L2: 0.1}}   & \multicolumn{1}{c|}{0.76} & 0.66  \\ \midrule
7  & \multicolumn{1}{c|}{\makecell{L0: 0.0 \\ L1: 0.0 \\ L2: 0.0}}   & \multicolumn{1}{c|}{0.00} & 0.00 & \multicolumn{1}{c|}{\makecell{L0: 0.85 \\ L1: 0.85 \\ L2: 0.3}} & \multicolumn{1}{c|}{0.65} & 0.35 & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.65 \\ L2: 0.4}} & \multicolumn{1}{c|}{0.62} & 0.22 & \multicolumn{1}{c|}{\makecell{L0: 0.95 \\ L1: 0.65 \\ L2: 0.15}} & \multicolumn{1}{c|}{0.34} & 0.19  \\ \midrule
8  & \multicolumn{1}{c|}{\makecell{L0: 0.4 \\ L1: 0.0 \\ L2: 0.0}}   & \multicolumn{1}{c|}{0.00} & 0.00 & \multicolumn{1}{c|}{\makecell{L0: 0.65 \\ L1: 0.4 \\ L2: 0.35}} & \multicolumn{1}{c|}{0.65} & 0.30 & \multicolumn{1}{c|}{\makecell{L0: 0.7 \\ L1: 0.7 \\ L2: 0.5}}   & \multicolumn{1}{c|}{0.62} & 0.12 & \multicolumn{1}{c|}{\makecell{L0: 0.5 \\ L1: 0.25 \\ L2: 0.2}}   & \multicolumn{1}{c|}{0.34} & 0.14  \\ \midrule
9  & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.05 \\ L2: 0.05}} & \multicolumn{1}{c|}{0.55} & 0.50 & \multicolumn{1}{c|}{\makecell{L0: 0.9 \\ L1: 0.2 \\ L2: 0.2}}   & \multicolumn{1}{c|}{0.79} & 0.59 & \multicolumn{1}{c|}{\makecell{L0: 0.7 \\ L1: 0.5 \\ L2: 0.5}}   & \multicolumn{1}{c|}{0.62} & 0.12 & \multicolumn{1}{c|}{\makecell{L0: 0.8 \\ L1: 0.7 \\ L2: 0.7}}    & \multicolumn{1}{c|}{0.46} & -0.24 \\ \midrule
10 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.1 \\ L2: 0.1}}   & \multicolumn{1}{c|}{0.67} & 0.57 & \multicolumn{1}{c|}{\makecell{L0: 1.0 \\ L1: 0.45 \\ L2: 0.45}} & \multicolumn{1}{c|}{0.81} & 0.36 & \multicolumn{1}{c|}{\makecell{L0: 0.85 \\ L1: 0.6 \\ L2: 0.6}}  & \multicolumn{1}{c|}{0.81} & 0.21 & \multicolumn{1}{c|}{\makecell{L0: 0.9 \\ L1: 0.55 \\ L2: 0.55}}  & \multicolumn{1}{c|}{0.65} & 0.10  \\ \midrule
\end{tabular}
\end{table*}

